Unstructured Overlapping Mesh Distribution in Parallel

We present a simple mathematical framework and API for parallel mesh and data distribution, load balancing, and overlap generation. It relies on viewing the mesh as a Hasse diagram, abstracting away information such as cell shape, dimension, and coordinates. The high level of abstraction makes our interface both concise and powerful, as the same algorithm applies to any representable mesh, such as hybrid meshes, meshes embedded in higher dimension, and overlapped meshes in parallel. We present evidence, both theoretical and experimental, that the algorithms are scalable and efficient. A working implementation can be found in the latest release of the PETSc libraries.

==> tikzlibraryquadtree.code.tex <==
% This file defines macros for making quadtree diagrams in tikz pictures.
% It depends on the tikz library for trees, so you file must include
%
% \usetikzlibrary{trees}
% \usetikzlibrary{quadtree}

% This puts a quadrant centered at the current location.
\def\quadrant{+(-1cm,-1cm) rectangle +(1cm,1cm) (0,0)}

% Morton order growth function
\tikzstyle{morton order}=[growth function=\quadtree@morton,
                          level distance=\quadtree@sqrt2,
   edge from parent path={(\tikzparentnode.center) (\tikzchildnode.center)}]

% Three options that control the placement of leaves

% Places space between leaves: the space is the same at each level, so this only
% works if the size of the leaves is less than the absolute space
\tikzset{quadtree absolute space/.initial=0.0}
% Places space between leaves proportional to the size of the leaves
\tikzset{quadtree relative space/.initial=0.0}
% Shrinks a leaf towards its center (after applying the above spaces)
\tikzset{quadtree scale/.initial=1.0}

\def\quadtree@morton{%
  \ifnum\tikznumberofcurrentchild=1\relax%
    \c@pgf@counta=-135\relax%
  \else\ifnum\tikznumberofcurrentchild=2\relax%
    \c@pgf@counta=-45\relax%
  \else\ifnum\tikznumberofcurrentchild=3\relax%
    \c@pgf@counta=135\relax%
  \else%
    \c@pgf@counta=45\relax%
  \fi\fi\fi
  \pgftransformscale{.5*(1-2^(\the\tikztreelevel-1)*%
(\pgfkeysvalueof{/tikz/quadtree absolute space})-%
(\pgfkeysvalueof{/tikz/quadtree relative space}))}%
  \pgftransformshift{\pgfpointpolar{\the\c@pgf@counta}%
  {\quadtree@sqrt2 * (2 - (1 -2^(\the\tikztreelevel-1)*%
(\pgfkeysvalueof{/tikz/quadtree absolute space})-%
(\pgfkeysvalueof{/tikz/quadtree relative space})))/%
(1-2^(\the\tikztreelevel-1)*(\pgfkeysvalueof{/tikz/quadtree absolute space})-
(\pgfkeysvalueof{/tikz/quadtree relative space}))}}
  \pgftransformscale{(\pgfkeysvalueof{/tikz/quadtree scale})}
}

\def\quadtree@sqrt2{1.41421356237310 cm}

% Example usage:
%
%  \draw [morton order,quadtree absolute space=0.05] coordinate
%    child {[red]\quadrant}
%    child {[green]\quadrant}
%    child {
%      child {[green]\quadrant}
%      child {
%        child {[green]\quadrant}
%        child {[blue]\quadrant}
%        child {[red]\quadrant}
%        child {[green]\quadrant}}
%      child {
%        child {[green]\quadrant}
%        child {[blue]\quadrant}
%        child {
%          child {[green]\quadrant}
%          child {[blue]\quadrant}
%          child {[red]\quadrant}
%          child {[green]\quadrant}}
%        child {[green]\quadrant}}
%      child {[red]\quadrant}
%      child {[green]\quadrant}}
%    child {[blue]\quadrant};

